Exascale Simulations of Fusion and Fission Systems

We discuss pioneering heat and fluid flow simulations of fusion and fission energy systems with NekRS on exascale computing facilities, including Frontier and Aurora. The Argonne-based code, NekRS, is a highly-performant open-source code for the simulation of incompressible and low-Mach fluid flow, heat transfer, and combustion with a particular focus on turbulent flows in complex domains. It is based on rapidly convergent high-order spectral element discretizations that feature minimal numerical dissipation and dispersion. State-of-the-art multilevel preconditioners, efficient high-order time-splitting methods, and runtime-adaptive communication strategies are built on a fast OCCA-based kernel library, libParanumal, to provide scalability and portability across the spectrum of current and future high-performance computing platforms. On Frontier, Nek5000/RS has achieved an unprecedented milestone in breaching over 1 trillion degrees of freedom with the spectral element methods for the simulation of the CHIMERA fusion technology testing platform. We also demonstrate for the first time the use of high-order overset grids at scale.

==> tex/rules.tex <==



Abstract

(150 word max)

Justification for ACM Gordon Bell Prize

(50 word max)

indicate what implementation or performance “high watermark” was achieved
(rather than the science that was enabled)

Performance Attributes

(use a table listing each attribute title and value in a separate row)

Category of achievement (1+ of:  scalability, time-to-solution, peak
performance)

Type of method used (1 of:  explicit, implicit, both explicit and implicit,
semi-implicit, n/a)

Results reported on the basis of (1 of:  whole application including I/O; whole
application except I/O; kernel only; other [specify])

Precision reported (1 of:  single precision, double precision, mixed precision)

System scale (1 of:  results measured on full-scale system, projected from
results of smaller system, other [specify])

Measurement mechanism (1 of:  timers, FLOP count, static analysis tool,
performance modeling, other [specify] )

Overview of the Problem

description of the problem and its importance, in terms understandable to a
non-specialist (1 p max)

Current State of the Art

quantitative discussion of current SoA, with emphasis on performance-related
aspects  (1 p max)

Innovations Realized

what the innovations are and how they were achieved (2 pp max)

How Performance Was Measured

(Note that preference is given to performance actually measured [not
projected], based on the entire application [including I/O] and with uniform
precision.  Explain in detail if any portion of total runtime was not included
in the measurements, if and where different precisions were used, or any
attributes listed in Section 3 as “other”).

what application(s) was used to measure performance (1 p max)

system and environment where performance was measured (1 p max)

Performance Results

include scalability (weak and strong), time to solution, efficiency (of
bottleneck resources), and peak performance (2 pp max)

Implications

implications for future systems and applications (1 p max)

References  (1 p max)

The committee will select up to 6 nominations as “finalists” made on the basis
of empirical performance measurements submitted (not extrapolated performance
predictions).  Each nominator should be prepared to reproduce both performance
and scientific results.

Finalist submission will be published in the SC proceedings and presented at
the SC conference.   Prior to publication, finalists will be allowed to correct
typographic errors, but no other changes to the text will be permitted prior to
publication unless specifically requested by the committee.




==> tex/tab2f.tex <==


\begin{table*}
\centering
\caption{CHIMERA Cases: nelv=\# of fluid elements; nelt=\# of thermal-fluid elements}
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\textbf{$E$} & \textbf{N} & \textbf{Type} & \textbf{dt} & \textbf{avg CFL} & \textbf{avg Pr} & \textbf{flops/rank} & \textbf{note} \\
\hline
  21M & 3 & overset & $1 \times 10^{-5}$ & 0.068 & 1          & 1001-2000 & \\ \hline
  21M & 4 & overset & $1 \times 10^{-5}$ & 0.112 & 1.046      & 1001-2000 & \\ \hline
  21M & 5 & overset & $1 \times 10^{-5}$ & 0.165 & 1.007      & 1001-2000 & \\ \hline
  21M & 5 & overset & $1 \times 10^{-4}$ & 1.483 & 1.046      & 1001-2000 & \\ \hline
  51M & 7 & fluid only & $1 \times 10^{-5}$ & 0.534 & 1       & 1001-2000 & \\ \hline
 211M & 7 & fluid only & $2 \times 10^{-4}$ & 1.087 & 5.216   & 1001-2000 & \\ \hline
%1.69B & 3 & fluid only & $1 \times 10^{-4}$ & 0.253 & 6.231  & 10001-15000 & \\ \hline
1.69B & 3 & fluid only & $5 \times 10^{-4}$ & 1.257 & 8.099   & 1001-2000 & pproj=8 \\ \hline
1.69B & 3 & fluid only & $5 \times 10^{-4}$ & 1.257 & 7.269   & 1001-2000 & pproj=L30 \\ \hline
1.69B & 7 & fluid only & $1 \times 10^{-4}$ & 1.103 & 50.195  & 101-300 & MG7531-cheb6 \\ \hline
1.69B & 9 & fluid only & $5 \times 10^{-5}$ & 0.872 & 120.55  & 21-60 & MG951-cheb3 \\ \hline
%1.69B & 9 & fluid only & $5 \times 10^{-5}$ & 0.872 & 68.725 & 21-60 & MG9751-cheb6 very slow \\ \hline
\end{tabular}
\label{tab:neknek2}
\end{table*}


